Learning a Latent Simplex in Input-Sparsity Time

We consider the problem of learning a latent $k$-vertex simplex $K\subset\mathbb{R}^d$, given access to $A\in\mathbb{R}^{d\times n}$, which can be viewed as a data matrix with $n$ points that are obtained by randomly perturbing latent points in the simplex $K$ (potentially beyond $K$). A large class of latent variable models, such as adversarial clustering, mixed membership stochastic block models, and topic models can be cast as learning a latent simplex. Bhattacharyya and Kannan (SODA, 2020) give an algorithm for learning such a latent simplex in time roughly $O(k\cdot\textrm{nnz}(A))$, where $\textrm{nnz}(A)$ is the number of non-zeros in $A$. We show that the dependence on $k$ in the running time is unnecessary given a natural assumption about the mass of the top $k$ singular values of $A$, which holds in many of these applications. Further, we show this assumption is necessary, as otherwise an algorithm for learning a latent simplex would imply an algorithmic breakthrough for spectral low rank approximation. At a high level, Bhattacharyya and Kannan provide an adaptive algorithm that makes $k$ matrix-vector product queries to $A$ and each query is a function of all queries preceding it. Since each matrix-vector product requires $\textrm{nnz}(A)$ time, their overall running time appears unavoidable. Instead, we obtain a low-rank approximation to $A$ in input-sparsity time and show that the column space thus obtained has small $\sin\Theta$ (angular) distance to the right top-$k$ singular space of $A$. Our algorithm then selects $k$ points in the low-rank subspace with the largest inner product with $k$ carefully chosen random vectors. By working in the low-rank subspace, we avoid reading the entire matrix in each iteration and thus circumvent the $\Theta(k\cdot\textrm{nnz}(A))$ running time.

==> preamble.tex <==
%\documentclass[11pt,letterpaper]{article}
%\usepackage{fullpage}


\newcommand{\ignore}[1]{}


\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\b{\mathbf{b}}
\def\MM{\mathbf{M}}
\def\HH{\mathbf{H}}
\def\Om{\mathbf{\Omega}}
\def\NN{\mathbf{N}}
\def\LL{\mathbf{L}}
\def\WW{\mathbf{W}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\II{\mathbb{I}}
\def\YY{\mathbf{Y}}
\def\XX{\mathbf{X}}
\def\PP{\mathbf{P}}
\def\pp{\mathbf{p}}
\def\UU{\mathbf{U}}
\def\uu{\mathbf{u}}
\def\VV{\mathbf{V}}
\def\EE{\mathbf{E}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\WW{\mathbf{W}}
\def\PI{\mathbf{\Pi}}
\def\QQ{\mathbf{Q}}
\def\GG{\mathbf{G}}
\def\MM{\mathbf{M}}
\def\mm{\mathbf{m}}
\def\ZZ{\mathbf{Z}}
\def\RR{\mathbf{R}}
\def\II{\mathbf{I}}
\def\Y{\mathbf{Y}}
\def\X{\mathcal{X}}
\def\S{\mathcal{S}}
\def\I{\mathcal{I}}
\def\R{\mathcal{R}}
\def\T{\mathcal{T}}

\def\cK{\mathcal{K}}



\def\prox{{\bf Proximate ~Latent Points~}}
\def\wellsep{{\bf Well Separatedness}}
\def\bU{{\bf U}}
\def\bV{{\bf V}}
\def\bI{{\bf I}}
\def\bX{{\bf X}}
\def\bp{{\bf q}}
\def\bq{{\bf p}}
\def\bu{{\bf u}}
\def\bv{{\bf v}}
\def\bx{{\bf x}}
\def\bw{{\bf w}}
\def\by{{\bf y}}
\def\bz{{\bf z}}
\def\bM{{\bf M}}
\def\bA{{\bf A}}
\def\bP{{\bf P}}
\def\bW{{\bf W}}
\def\bB{{\bf B}}
\def\Var{\mbox{Var}}
\def\var{\mbox{Var}}
\def\Null{\mbox{Null}}
\def\Span{\mbox{Span}}
\def\Proj{\mbox{Proj}}
\def\bQ{{\bf Q}}
\def\bE{{\bf E}}
\def\bR{{\bf R}}
\def\bF{{\bf F}}
\def\bG{{\bf G}}
\def\bR{{\bf R}}
\def\bS{{\bf S}}


\def\BAD{\hbox{BAD}}
\def\for{\hbox{ for }}

\def\Var{\mbox{Var}}
\def\Max{\mbox{Max}}
\def\Min{\mbox{Min}}
\def\prob{\hbox{Pr}}
\def\proj{\mbox{Proj}}
\def\Proj{\mbox{Proj}}
\def\nnz{\textsf{nnz}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\dx}{\;\mathrm{d}x}
\newcommand{\dy}{\;\mathrm{d}y}

\def\Sig{\mathbf{\Sigma}}
\newcommand\SLASH{\char`\\}

\def\Lam{\mathbf{\Lambda}}
\usepackage{ amssymb }

\newcommand\bb[1]{\textsc{\textbf{#1}}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}

\def\poly{\textrm{poly}}

\def\probf#1#2{\mbox{\bf Pr}_{#1}\left[ #2 \right]}
\def\prob#1#2{\mbox{\bf Pr}_{#1}\left[ #2 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\bf \mathbb{E}}_{#1}[ #2 ]}
\def\expecf#1#2{{\bf \mathbb{E}}_{#1}\left[ #2 \right]}
\def\var#1{\mbox{\bf Var}[ #1 ]}
\def\varf#1{\mbox{\bf Var}\left[ #1 \right]}


\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}

\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\trs#1{\mathrm{Tr}_{\sigma} \left(#1 \right)}


\def\floor#1{\left\lfloor #1 \rightloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\abs#1{\left|#1  \right|}

\def\norm#1{\left\| #1 \right\|}
\def\smallnorm#1{\| #1 \|}




\DeclareRobustCommand{\bbone}{\text{\usefont{U}{bbold}{m}{n}1}}

\DeclareMathOperator{\EX}{\mathbb{E}}% expected value
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}



\def\C{{\mathcal{Y}}}
\def\OPT{{\mathcal{OPT}}}
\def\expec#1#2{{\bf \mathbb{E}}_{#1}[ #2 ]}
\def\expecf#1#2{{\bf \mathbb{E}}_{#1}\left[ #2 \right]}
\def\var#1{\mbox{\bf Var}[ #1 ]}
\def\varf#1{\mbox{\bf Var}\left[ #1 \right]}

\numberwithin{equation}{section}
\numberwithin{figure}{section}
\theoremstyle{plain}
	\newtheorem{theorem}{Theorem}[section]
	\newtheorem{thm}[theorem]{Theorem}
	\newtheorem{lem}[theorem]{Lemma}
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
 	\newtheorem{cor}[theorem]{Corollary}
	\newtheorem{fact}[theorem]{Fact}
	\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
	\newtheorem{definition}[theorem]{Definition}
	\newtheorem{defn}[theorem]{Definition}
	\newtheorem*{remark*}{Remark}

\usepackage[framemethod=TikZ]{mdframed}
\newcounter{Frame}
\newenvironment{Frame}[1][htb]{%
\refstepcounter{Frame}
    \begin{mdframed}[%
        frametitle={#1},
        skipabove=\baselineskip plus 2pt minus 1pt,
        skipbelow=\baselineskip plus 2pt minus 1pt,
        linewidth=1.0pt,
        frametitlerule=true,
        nobreak=true
    ]%
}{%
    \end{mdframed}
}
\newtheorem{asm}{Assumption}


==> subspace.tex <==
\section{Closeness of Subspaces and Subspace power iteration}\label{subspace}
In this section we will present the classical Subspace power iteration algorithm
which finds an approximation to the subspace spanned by the top $k$ (left) singular vectors
of $\bA$. It has a well-known elegant proof of convergence, which also we present here, since,
usual references often present more general (and also more complicated) proofs. Let
$$\mbox{SVD}(\bA)=\sum_{t=1}^ds_t(\bA) v_tu_t^T.$$

%
\subsection{Closeness of Subspaces}
First, we recall a measure of closeness of sub-spaces.
Numerical Analysis has developed, namely, the notion of angles between sub-spaces, called Principal
angles. Here, we need only one of the principal angles which we define now.

For any two sub-spaces $F,F'$ of ${\bf R}^d$, define
$$\sin\Theta(F,F')=\Max_{u\in F}\Min_{v\in F'} \sin\theta (u,v)=\Max_{u\in F, |u|=1}\Min_{v\in F'}|u-v|.$$
$$  \cos\Theta(F,F')=\sqrt{ 1-\sin\Theta^2(F,F')}.$$
The following are known facts about $\sin\Theta$ function:
If $F,F'$ have the same dimension and the columns of
$\bF$ (respectively $\bF'$) form an orthonormal basis of $F$ (respectively $F'$), then
\begin{eqnarray}\label{cos-F-F-prime}
\cos\Theta(F,F')& =s_{\text{Min}}(\bF^T\bF')\nonumber \\
\cos\Theta(F',F) & =\cos\Theta(F,F')\nonumber\\
\tan\Theta(F,F') &=||\bG^T\bF'(\bF^T\bF')^{-1}||,
\end{eqnarray}
where, the columns of matrix $\bG$ form a basis for $F^\perp$, and assuming the inverse of $\bF^T\bF'$ exists.

An important Theorem due to Wedin\citep{wedin72}, also known as the $\sin\Theta$ theorem, proves a bound on the $\sin\Theta$ between SVD-subspaces of a matrix and its perturbation:

\begin{theorem}\citep{wedin72}\label{wedin}
Suppose $\bR,\bS$ are any two $d\times n$ matrices. Let $m\leq \ell$ be any two positive integers. 
Let $S_m(\bR),S_\ell (\bS)$ denote respectively the subspaces spanned by the top $m$, respectively top $\ell$ left singular vectors of $\bR$, respectively,
$\bS$. 
Suppose $\gamma =s_m(\bR)-s_{\ell+1}(\bS) >0$. 
Then,
$$\sin\Theta (S_m(\bR),S_\ell (\bS))\leq \frac{||\bR-\bS||}{\gamma}.$$
\end{theorem}
%
Corollary below says the SVD subspace of $\bA$ is approximately equal to the Span of $\bP$.
\begin{corollary}\label{wedin-2}
Let $\bA,\bP$ be defined in Section ~\ref{sec:lks}.
$$\sin\Theta(\Span(v_1,v_2,\ldots ,v_k),\Span(\bP))\leq\frac{||\bA-\bP||}{s_k(\bA)}. $$
\end{corollary}
\begin{proof}
Apply Theorem (\ref{wedin}) with $\bR=\bA,\bS=\bP,m=\ell=k$
\end{proof}
We next find SVD subspace of $\bA$ by subspace power iteration.

\subsection{Subspace-Power Iteration}\label{power-method}

\begin{algorithm}[h]
\caption{{Subspace Power Method}}\label{alg:spm}
\begin{algorithmic}
\Function{{\tt Subspace-Power}}{$\bA$, $T$}
\State \textbf{Input}:$\bA$ and $T$ \Comment{T is the number of iterations}
\State \emph{Initialize:} $Q_0$ be a random $d\times k$ matrix with orthonormal columns.

\ForAll{$t=1,2,\ldots,  T$}
\State Set ${\bf Z_{t}}= \bA\bA^T {\bf Q_{t-1}}.$
\State Do Grahm-Schmidt on ${\bf Z_{t}}$ to obtain ${\bf Q_t}$
\EndFor

\Return ${\bf Q_{T}}$. $V=\Span({\bf Q_T})$.
\EndFunction
\end{algorithmic}
\end{algorithm}


Recall that $v_1,\ldots,v_d$ are left singular vectors of $\bA$ and
$\bQ_T$ is the $T$ iterate of the subspace power iteration.
\begin{theorem}\label{convergence-power}
{\bf Convergence of Subspace power iteration}
\begin{equation}\label{power-iteration}
\sin\Theta (\Span(v_1,v_2,\ldots ,v_k), \Span ({\bf Q_{c\ln d}}))   \leq \frac{\alpha^2}{1000k^9}.
\end{equation}
\end{theorem}
\begin{proof}
Let ${\bf F},{\bf G}$ be the $d\times k,d\times (d-k)$ matrices with columns $v_1,v_2,\ldots ,v_k$, respectively
$v_{k+1},v_{k+2},\ldots ,v_d$ and $F,G$ be respectively the subspaces spanned by their columns.
Note that from (\ref{cos-F-F-prime}), we have
$$\tan\Theta(F, Q_t)=||{\bf G}^T{\bf Q_t}\left( \bF^T{\bf Q_t}\right)^{-1}||.   $$
\begin{lemma}
$$\tan\Theta(F, Q_t)\leq \left( \frac{s_{k+1}(\bA)}{s_k(\bA)}\right)^{2t}||{\bf G}^T{\bf Q_0}\left( \bF^T{\bf Q_0}\right)^{-1}||.$$
\end{lemma}
\begin{proof}
${\bf Q_t}={\bf Z_t}{\bf R}$, where $\bR$ is the invertiblke matrix of Grahm-Scmidt orthogonalization, We write

Define $DS_{i:j} = \mbox{Diag}(s_{i}^{2}(\bA),s_{i+1}^{2}(\bA),\ldots s_j(\bA)^{2})$ for positive integers $i,j$ such that $i < j$.
\begin{align*}
&||{\bf G}^T{\bf Q_t}\left( \bF^T{\bf Q_t}\right)^{-1}||=||{\bf G}^T{\bf Z_t}\bR\bR^{-1}\left( \bF^T{\bf Z_t}\right)^{-1}||  \\
&=||DS_{k+1:d} {\bf G}^T{\bf Q_{t-1}}\left( F^T{\bf Q_{t-1}}\right)^{-1}
DS_{1:k}^{-1}||\\
&\leq \frac{s_{k+1}^2}{s_k^2}||{\bf G}^T{\bf Q_{t-1}}\left( \bF^T{\bf Q_{t-1}}\right)^{-1}||   ,
\end{align*}
since, $\bG^T{\bf Z_t}=\bG^T\bA\bA^T{\bf Q_{t-1}}=\bG^T\sum_{t=1}^ds_t^2(\bA)v_tv_t^T{\bf Q_{t-1}}=DS_{k+1:d}\bG^T{\bf Q_{t-1}}$
and similarly, $\bF^T{\bf Z_t}=DS_{1:k}\bF^T{\bf Q_{t-1}}$. This proves the Lemma by induction on $t$.
\hfill\end{proof}
We prove in Claim ~\ref{singular-P-M} that $s_k(\bP)\geq 4\sigma\sqrt n$. Also, $s_{k+1}(\bA)\leq s_{k+1}(\bP)+||\bA-\bP||
=\sigma\sqrt n$. Thus, we have
$s_{k+1}/s_k\leq 1/2$ and now applying Lemma above, Theoirem (\ref{convergence-power}) follows,
since for a random choice of ${\bf Q_0}$, we have $||{\bf G}^T{\bf Q_0}\left( \bF^T{\bf Q_0}\right)^{-1}||\leq \mbox{poly}(nd)$.
\hfill\end{proof}

Next, we apply Wedin's theorem to
prove Lemma (\ref{sin-theta}) below which
says
that any $k$ dimensional space $V$ with small $\sin\Theta$ distance to Span$(v_1,v_2,\ldots ,v_k)$ also has small
$\sin\Theta$ distance to Span$(\bM)$. We first need a technical Claim.

\begin{claim}\label{singular-P-M}
Recall that $s_t$ denotes the $t$ th singular value.
$$s_k(\bM)\geq\frac{1000k^{8.5}}{\alpha^2}\frac{\sigma}{\sqrt\delta}\; ;\; s_k(\bP)\geq \frac{995k^{8.5}\sqrt n}{\alpha^2}\sigma.$$
\end{claim}
\begin{proof}
$s_k(\bM)=\Min_{x:|x|=1} |Mx|$. For any $x, |x|=1$, there must be an $\ell$ with $|x_\ell|\geq 1/\sqrt k$.
Now, $|\bM x|\geq |proj(\bM x, \Null(\bM\setminus M_{\cdot,\ell}))|=|x_\ell | |proj(M_{\cdot,\ell}, \Null(\bM\setminus M_{\cdot,\ell}))|
\geq \alpha |M_{\cdot,\ell}|/\sqrt k\geq 1000k^9\sigma/(\alpha^2\sqrt\delta \sqrt k)$ by (\ref{condition-number-100}) and (\ref{spectral-bound})
proving the first assertion of the Claim.

Now, we prove the second.
Recall there are sets $S_1,S_2,\ldots ,S_k\subseteq [n]$ with $\forall j\in S_\ell, |P_{\cdot,j}-M_{\cdot,\ell}|\leq \frac{4\sigma}{\sqrt\delta}$.
We claim the $S_\ell$ are disjoint: if not, say, $j\in S_\ell\cap S_{\ell'}$. Then, $|P_{\cdot,j}-M_{\cdot,\ell}|, |P_{\cdot,j}-M_{\cdot,\ell'}|
\leq 4\sigma/\sqrt\delta$ implies $|M_{\cdot,\ell}-M_{\cdot,\ell'}|\leq 8\sigma/\sqrt\delta\leq \alpha^2\Min_\ell|M_{\cdot,\ell}|/100k^9$
by (\ref{spectral-bound}). But, by (\ref{condition-number-100}), $|M_{\cdot,\ell}-M_{\cdot,\ell'}|\geq |\proj(M_{\cdot,\ell},\Null(\bM\setminus M_{\cdot,\ell})|
\geq\alpha |M_{\cdot,\ell}|$ producing a contradiction.

Let $\bP'$ be a $d\times k\delta n$ sub-matrix of $\bP$ with its columns $j\in S_1\cup S_2\cup\ldots \cup S_k$ and let $\bM'$ be the
$d\times k\delta n$ matrix with $M'_{\cdot,j}=M_{\cdot,\ell}$ for all $j\in S_\ell, \ell=1,2,\ldots ,k$. We have $s_k(\bM')\geq \sqrt{\delta n}s_k(\bM)
\geq 1000k^{8.5}\sqrt n\sigma/\alpha^2$. Now, $||\bP'-\bM'||\leq \sqrt{k\delta n}4\sigma /\sqrt\delta$. Since
$s_k(\bP)\geq s_k(\bP')\geq s_k(\bM')-||\bP'-\bM'||$,
the second part of the claim follows.
\hfill\end{proof}

\begin{lemma}\label{sin-theta}
Let $v_1,v_2,\ldots ,v_k$ be the top $k$ left singular vectors of $\bA$.
Let $V$ be any $k-$ dimensional sub-space of ${\bf R}^d$ with
$$\sin\Theta(V,\Span(v_1,v_2,\ldots ,v_k))\leq\frac{\alpha^2}{1000k^9}.$$

For every unit length vector $x\in V$, there is a vector $y\in \Span(\bM)$
with $$|x-y|\leq \frac{\alpha^2}{500k^{8.5}}.$$
\end{lemma}
\begin{proof}
Since $\Span (\bP)\subseteq \Span(\bM)$, it suffices to prove the Lemma with $y\in$ Span$(\bP)$.
Corollary ~\ref{wedin-2} implies:
$$\mbox{ Sin }\Theta\left( \Span(v_1,v_2,\ldots v_k), \mbox{Span}(\bP)\right)
\leq $$
$$\frac{||\bA-\bP||}{s_k(\bA)}\leq \frac{||\bA-\bP||}{s_k(\bP)-||\bA-\bP||}\leq \frac{\sigma}{(995k^{8.5}\sigma/\alpha^2)-\sigma}\leq \frac{\alpha^2}{994k^{8.5}}.$$

Now, $\sin\Theta(V,\Span(v_1,v_2,\ldots ,v_k))\leq\alpha^2/1000k^9$ and,
$\sin\Theta (V,\Span(\bM))\leq \sin\Theta(V,\Span(v_1,v_2,\ldots ,v_k)) +\sin\Theta( \Span(v_1,v_2,\ldots ,v_k),\Span(\bM))$,
which together imply the Lemma. [We have used here the triangle inequality for $\sin\Theta$ which follows directly from the definition
of $\sin\Theta$.]
\hfill\qed
\end{proof}

